Correctness and Fairness of Tendermint-core Blockchains

Tendermint-core blockchains (e.g. Cosmos) are considered today one of the most viable alternatives for the highly energy consuming proof-of-work blockchains such as Bitcoin and Ethereum. Their particularity is that they aim at offering strong consistency (no forks) in an open system combining two ingredients (i) a set of validators that generate blocks via a variant of Practical Byzantine Fault Tolerant (PBFT) consensus protocol and (ii) a selection strategy that dynamically selects nodes to be validators for the next block via a proof-of-stake mechanism. However,the exact assumptions on the system model under which Tendermint underlying algorithms are correct and the exact properties Tendermint verifies have never been formally analyzed. The contribution of this paper is two-fold. First, while formalizing Tendermint algorithms we precisely characterize the system model and the exact problem solved by Tendermint. We prove that in eventual synchronous systems a modified version of Tendermint solves (i) under additional assumptions, a variant of one-shot consensus for the validation of one single block and (ii) a variant of the repeated consensus problem for multiple blocks. These results hold even if the set of validators is hit by Byzantine failures, provided that for each one-shot consensus instance less than one third of the validators is Byzantine. Our second contribution relates to the fairness of the rewarding mechanism. It is common knowledge that in permisionless blockchain systems the main threat is the tragedy of commons that may yield the system to collapse if the rewarding mechanism is not adequate. Ad minimum the rewarding mechanism must be fair, i.e.distributing the rewards in proportion to the merit of participants. We prove, for the first time in blockchain systems, that in repeated-consensus based blockchains there exists an (eventual) fair rewarding mechanism if and only if the system is (eventual) synchronous. We also show that the original Tendermint rewarding is not fair, however, a modification of the original protocol makes it eventually fair.

==> proofFairness.tex <==
% !TeX root = main.tex

\begin{lemma}\label{l:tendermintNotFair}
	The reward mechanism of Tendermint is not eventually fair.
\end{lemma}

\begin{proofL}%[Proof of Lemma \ref{l:tendermintNotFair}]
	We assume that the system becomes synchronous, and that $\TimeOutCommit < \Delta$, where $\Delta$ is the maximum message delay in the network. 
	For any height $H$, let $p_i$ be a validator for the height $H-1$ and $p_j$ the validator whose proposal get decided for the height $H$.
	It may happen that $p_j$ did not receive the commit from $p_i$ before proposing its block.
	Hence when the block is decided, $p_i$ does not get a reward for its effort, which contradicts the condition \ref{fairness4bis} of the reward mechanism fairness.
	The Tendermint's reward mechanism is not eventually fair.
	\renewcommand{\toto}{l:tendermintNotFair}
\end{proofL}

\begin{lemma}\label{l:tendermintModFair}
	The variant of the Tendermint's reward mechamism where the $\TimeOutCommit$ increases for each round until it catches up the message delay, called the Tendermint's reward mechanism with modulable timeouts, is eventually fair. 
\end{lemma}
\begin{proofL}%[Proof of Lemma \ref{l:tendermintModFair}]
	We change the reward mechanism in Tendermint  as follows: %, for the height $H$
	\begin{itemize}
		\item Once a new block is decided, say for height $H$, processes wait for at most \TimeOutCommit to collect the decision from the other validators for that height, and put them in their set $\toReward$.
		\item If a process did not get the commits from all the validators for that height before the expiration of the time-out, it increases the time-out for the next height.
		\item During the consensus at height $H$, let us assume that $p_i$ proposes the block that will get decided in the consensus. $p_i$ gives the reward to the processes in its $\toReward$. 
	\end{itemize}
	In this reward mechanism, \TimeOutCommit is increased whenever a process does not have the time to deliver all the commits for the previous round.
	We prove that this reward mechanism is eventually fair.
	
	There is a point in time $t$ from when the system will become synchronous, and all the commits will be delivered by correct processes before the next height.
	From the time $t$, at height $H$ all correct processes know the exact set of validators that committed the block from $H-1$, and they give to those validators from $H-1$ a reward parameter greater than $0$.
	The validators in $H$  give the reward to the validators that committed and which are the only one with a reward parameter greater than $0$ for $H-1$, which satisfy the fairness conditions \ref{fairness1}, \ref{fairness2} %, \ref{fairness3} 
	and \ref{fairness4bis}, so the reward mechanism presented is eventually fair.
	\renewcommand{\toto}{l:tendermintModFair}
\end{proofL}

\begin{theorem}\label{t:tendermintFair}
	In an eventual synchronous system, if the selection mechanism is fair, then the Tendermint Repeated Consensus with the reward mechanism with modulable time-outs, is eventually fair.
\end{theorem}
\begin{proofT}%[Proof of Theorem \ref{t:tendermintFair}]
	The proof follows by Lemma \ref{l:tendermintModFair}.
	\renewcommand{\toto}{t:tendermintFair}
\end{proofT}


\begin{theorem}\label{t:strongFairness}
		There exists a fair reward mechanism in a Repeated Consensus based blockchain protocol iff the system is synchronous.
	\end{theorem}
\begin{proofT}%[Proof of Theorem \ref{t:strongFairness}]
	We prove this theorem by double implication.
	\begin{itemize}
		\item If the system is synchronous, then there exists a fair reward mechanism.
			
			We assume that the system is synchronous and all messages are delivered before the $x$ following blocks. We consider the following reward mechanism.
			For all the correct validators at any height $H$, if $H-x \le 0$, do not reward yet, otherwise:
			\begin{itemize}
				%\item Wait for receiving the messages from validators for the block $H-x$ before starting the block $H$, 
				\item Set to $1$ the reward parameters of all correct validators in $H-x$, and to $0$ the merit parameters of the others.
				\item Reward only the validators with a reward parameter equal to $1$ from the height $H-x$.
			\end{itemize}
			We prove in the following that the above reward mechanism is fair.
			
			Note that the system is synchronous and messages sent are delivered within at most $x$ blocks.
%				Since there is a consensus and that the set of validator for a block in the blockchain is known in advance, then only blocks in the blockchain will be considered by the correct validators in $H$. 
			Therefore, the exact set of correct validators at $H-x$ is known by all at $H$. 
			By construction, the validators in $H$ exactly give the reward to the correct validators who are the only one with a reward parameter for $H-x$ greater than $0$, which satisfies the fairness conditions (\ref{fairness1}, \ref{fairness2} %, \ref{fairness3} 
			and \ref{fairness4}).
			
%			This implication is a corollary of the lemma \ref{l:totalView}. 
%			In a synchronous system, all messages, from correct processes, are received before the end of the corresponding round, which means that the processes have a perfect view of the validators for any given block. By lemma \ref{l:totalView}, there exists a fair reward mechanism.
			
		\item If there exists a fair reward mechanism, then the system is synchronous.
			
			By contradiction, we assume that $\mathcal{P}$ is a protocol having a fair reward mechanism and that, the system is not synchronous.
			We say that the validators following $\mathcal{P}$ are the correct validators.
			%By condition \ref{fairness4}, we know that for a given block in the blockchain, all and only the processes that have a merit parameter different that $0$ for that block got a reward.
			Let $V^{i}$ be a set of validators for the height $i$, and $V^{j}, (j >i)$ be the set of validators who gave the reward to the correct validators in $V^i$. 
			Since the system is not synchronous, the validators in $V^{j}$ may not receive all messages from $V^{i}$ before giving the reward.
			
			By conditions \ref{fairness1}, and \ref{fairness2}, %and \ref{fairness3}, 
			it follows that all and only the correct validators in $V^i$ have a reward parameter greater than $0$.
			%Since $V^{j}$ is the set of validators who gives the reward to the correct processes in $V^{i}$, and 
			Since the reward mechanism is fair, with the condition \ref{fairness4}, we have the validators in $V^{j}$ gave the reward only to the correct validators in $V^i$. That means that the correct validators in $V^j$ know exactly who were the correct validators in $V^i$,
			so they got all the messages before giving the reward. Contradiction, which conclude the proof.
	\end{itemize}
	%There exists a fair reward mechanism iff the system is synchronous.
	\renewcommand{\toto}{t:strongFairness}
\end{proofT}

\begin{theorem}\label{t:eventualFairness}
	There exists an eventual fair reward mechanism in a Repeated Consensus based blockchain protocol iff the system is eventually synchronous or synchronous.
\end{theorem}
\begin{proofT}%[Proof of Theorem \ref{t:eventualFairness}]
	We proof this result by double implication.
	\begin{itemize}
		\item If the system is eventually synchronous or synchronous, then there exists an eventual fair reward mechanism.
			
			If the system is synchronous, the proof follows directly from theorem \ref{t:strongFairness}. Otherwise, we prove that the following reward mechanism is eventually fair.
			When starting the height $H$, the correct validator for $H$ do the following:
			\begin{itemize}
				\item Start the time-out for the reception of the messages from validators for the block $H-1$;
				\item Wait for receiving the messages from validators for the block $H-1$ or the time-out to expire.
					If the time-out expires before the reception of more that $2n/3$ of the messages, increase the time-out for the next time;
				\item Set to $1$ the reward parameters for $H-1$ of the correct validators which messages where received, and to $0$ the merit parameters of the others;
				\item Reward only the validators for the height $H-1$ which have a merit parameter different than $0$.
			\end{itemize}
			Since the system is eventually synchronous, eventually when the system will become synchronous, the processes, in particular the validators for $H$ will receive messages for all the correct validators from round $H-1$ before the round $H$.
			We note that the condition \ref{fairness4bis} is a weaker form of the condition \ref{fairness4} where we do not consider the beginning.
			So we end the proof by applying the theorem \ref{t:strongFairness} from the time when the system becomes synchronous.
			
		\item If there exists an eventual fair reward mechanism, then system is eventually synchronous or synchronous.
			
			If the reward mechanism is fair, by theorem \ref{t:strongFairness}, the communication is synchronous, which ends the proof.
			Otherwise, since the reward mechanism is eventually fair, then there is a point in time $t$ from when all the rewards are correctly distributed.
			By considering $t$ as the beginning of our execution, then we have that the reward mechanism is fair after $t$, so by the theorem \ref{t:strongFairness}, the system is synchronous from $t$.
			If the system were not synchronous before $t$, that means that it is eventually synchronous, otherwise, it is synchronous.
			Which ends the proof.
	\end{itemize}
	\renewcommand{\toto}{t:eventualFairness}
\end{proofT}

	\begin{corollary}\label{c:asyncFairness}
		In an asynchronous system, there is no (eventual) reward mechanism, so if the communication system is asynchronous, then there is no (eventual) fair Repeated Consensus-based Blockchain protocol.
		Note that this result is valid even if all the processes are correct.
	\end{corollary} 


==> related.tex <==
\paragraph{Tendermint}
	Tendermint Byzantine Fault Tolerant Consensus\cite{http://tendermint.readthedocs.io/en/master/specification/byzantine-consensus-algorithm.html}
	(Tendermint protocol) is a protocol that was proposed in \cite{paperTendermint} which aim to solve the consensus problem on Blockchains with limited energy consumption.
	We proof that it satisfies the consensus.
